Robust Contrastive Learning Using Negative Samples with Diminished Semantics

Unsupervised learning has recently made exceptional progress because of the development of more effective contrastive learning methods. However, CNNs are prone to depend on low-level features that humans deem non-semantic. This dependency has been conjectured to induce a lack of robustness to image perturbations or domain shift. In this paper, we show that by generating carefully designed negative samples, contrastive learning can learn more robust representations with less dependence on such features. Contrastive learning utilizes positive pairs that preserve semantic information while perturbing superficial features in the training images. Similarly, we propose to generate negative samples in a reversed way, where only the superfluous instead of the semantic features are preserved. We develop two methods, texture-based and patch-based augmentations, to generate negative samples. These samples achieve better generalization, especially under out-of-domain settings. We also analyze our method and the generated texture-based samples, showing that texture features are indispensable in classifying particular ImageNet classes and especially finer classes. We also show that model bias favors texture and shape features differently under different test settings. Our code, trained models, and ImageNet-Texture dataset can be found at https://github.com/SongweiGe/Contrastive-Learning-with-Non-Semantic-Negatives.

==> sections/archive.tex <==

\section{Class accuracy of models with $\alpha=0$ and $\alpha=2$}
\begin{table}[]
\begin{tabular}{lllll}
\toprule
finer class & coarse class & $\alpha=0$ & $\alpha=2$ &$\Delta$ accuracy \\
\midrule
American Staffordshire terrier & dog              & 60.66667 & 69.33333 & 8.666667 \\
Saluki                         & dog              & 68.66667 & 76.66667 & 8        \\
chime                          & instrument       & 60       & 67.33333 & 7.333333 \\
American coot                  & bird             & 84.66667 & 90.66667 & 6        \\
hognose snake                  & snake            & 75.33333 & 80.66667 & 5.333333 \\
rocking chair                  & furniture        & 62.66667 & 68       & 5.333333 \\
Chesapeake Bay retriever       & dog              & 66       & 71.33333 & 5.333333 \\
dung beetle                    & bug              & 82.66667 & 88       & 5.333333 \\
bottlecap                      & other            & 73.33333 & 78.66667 & 5.333333 \\
iron                           & tool             & 74.66667 & 80       & 5.333333 \\
mousetrap                      & technology       & 72       & 77.33333 & 5.333333 \\
slide rule                     & technology       & 73.33333 & 78.66667 & 5.333333 \\
pineapple                      & fruit            & 82       & 87.33333 & 5.333333 \\
hard disc                      & electronics      & 76       & 80.66667 & 4.666667 \\
mortarboard                    & hat              & 70       & 74.66667 & 4.666667 \\
purse                          & accessory        & 64       & 68.66667 & 4.666667 \\
toy terrier                    & dog              & 50       & 54.66667 & 4.666667 \\
throne                         & furniture        & 72.66667 & 77.33333 & 4.666667 \\
bonnet                         & hat              & 70       & 74       & 4        \\
tabby                          & cat              & 84.66667 & 88.66667 & 4        \\
red fox                        & wild dog         & 76       & 79.33333 & 3.333333 \\
stretcher                      & furniture        & 62.66667 & 66       & 3.333333 \\
papillon                       & dog              & 88.66667 & 92       & 3.333333 \\
walking stick                  & bug              & 80       & 83.33333 & 3.333333 \\
football helmet                & sports equipment & 88.66667 & 92       & 3.333333 \\
harmonica                      & instrument       & 74.66667 & 78       & 3.333333 \\
green mamba                    & snake            & 77.33333 & 80       & 2.666667 \\
borzoi                         & dog              & 80       & 82.66667 & 2.666667 \\
laptop                         & electronics      & 72       & 74.66667 & 2.666667 \\
tile roof                      & building         & 79.33333 & 82       & 2.666667 \\
stinkhorn                      & fungus           & 87.33333 & 90       & 2.666667 \\
modem                          & electronics      & 62.66667 & 65.33333 & 2.666667 \\
meerkat                        & mongoose         & 80.66667 & 83.33333 & 2.666667 \\
fiddler crab                   & crustacean       & 58       & 60       & 2        \\
boxer                          & dog              & 70       & 72       & 2        \\
leafhopper                     & bug              & 92.66667 & 94.66667 & 2        \\
gibbon                         & primate          & 83.33333 & 85.33333 & 2        \\
park bench                     & furniture        & 80.66667 & 82.66667 & 2        \\
safety pin                     & tool             & 53.33333 & 55.33333 & 2        \\
head cabbage                   & vegetable        & 82.66667 & 84.66667 & 2        \\
chocolate sauce                & food             & 74       & 76       & 2        \\
garter snake                   & snake            & 87.33333 & 88.66667 & 1.333333 \\
lorikeet                       & bird             & 95.33333 & 96.66667 & 1.333333 \\
standard poodle                & dog              & 81.33333 & 82.66667 & 1.333333 \\
wild boar                      & hog              & 91.33333 & 92.66667 & 1.333333 \\
goose                          & bird             & 84.66667 & 86       & 1.333333 \\
Walker hound                   & dog              & 73.33333 & 74.66667 & 1.333333 \\
boathouse                      & building         & 92       & 93.33333 & 1.333333 \\
computer keyboard              & electronics      & 78.66667 & 80       & 1.333333 \\
obelisk                        & building         & 82       & 83.33333 & 1.333333 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[]
\begin{tabular}{lllll}
\toprule
finer class & coarse class & $\alpha=0$ & $\alpha=2$ &$\Delta$ accuracy \\
\midrule
rotisserie                     & cooking          & 88.66667 & 90       & 1.333333 \\
rock crab                      & crustacean       & 68       & 68.66667 & 0.666667 \\
Rottweiler                     & dog              & 71.33333 & 72       & 0.666667 \\
Doberman                       & dog              & 71.33333 & 72       & 0.666667 \\
hare                           & rabbit           & 90       & 90.66667 & 0.666667 \\
Dutch oven                     & cooking          & 84       & 84.66667 & 0.666667 \\
lampshade                      & decor            & 79.33333 & 80       & 0.666667 \\
pickup                         & vehicle          & 87.33333 & 88       & 0.666667 \\
reel                           & technology       & 60.66667 & 61.33333 & 0.666667 \\
gyromitra                      & fungus           & 93.33333 & 94       & 0.666667 \\
milk can                       & container        & 62       & 62.66667 & 0.666667 \\
coyote                         & wild dog         & 78.66667 & 79.33333 & 0.666667 \\
cinema                         & building         & 78.66667 & 79.33333 & 0.666667 \\
little blue heron              & bird             & 93.33333 & 93.33333 & 0        \\
Chihuahua                      & dog              & 54.66667 & 54.66667 & 0        \\
bannister                      & furniture        & 86       & 86       & 0        \\
bassinet                       & furniture        & 84.66667 & 84.66667 & 0        \\
gasmask                        & accessory        & 82       & 82       & 0        \\
jean                           & clothing         & 76.66667 & 76.66667 & 0        \\
window screen                  & decor            & 74.66667 & 74.66667 & 0        \\
wing                           & other            & 93.33333 & 93.33333 & 0        \\
carbonara                      & food             & 89.33333 & 89.33333 & 0        \\
Mexican hairless               & dog              & 81.33333 & 80.66667 & -0.66667 \\
sarong                         & clothing         & 69.33333 & 68.66667 & -0.66667 \\
Gila monster                   & lizard           & 80       & 79.33333 & -0.66667 \\
garden spider                  & arachnid         & 96       & 95.33333 & -0.66667 \\
African hunting dog            & dog              & 100      & 99.33333 & -0.66667 \\
langur                         & primate          & 74       & 73.33333 & -0.66667 \\
car wheel                      & technology       & 72       & 71.33333 & -0.66667 \\
mixing bowl                    & cooking          & 92       & 91.33333 & -0.66667 \\
moped                          & vehicle          & 82.66667 & 82       & -0.66667 \\
pirate                         & person           & 94.66667 & 94       & -0.66667 \\
tripod                         & technology       & 68       & 67.33333 & -0.66667 \\
vacuum                         & electronics      & 68       & 67.33333 & -0.66667 \\
pedestal                       & furniture        & 75.33333 & 74       & -1.33333 \\
American lobster               & crustacean       & 94       & 92.66667 & -1.33333 \\
ski mask                       & clothing         & 81.33333 & 80       & -1.33333 \\
theater curtain                & decor            & 90       & 88.66667 & -1.33333 \\
Great Dane                     & dog              & 48       & 46.66667 & -1.33333 \\
robin                          & bird             & 90.66667 & 89.33333 & -1.33333 \\
ambulance                      & vehicle          & 96.66667 & 95.33333 & -1.33333 \\
cocktail shaker                & cooking          & 77.33333 & 76       & -1.33333 \\
honeycomb                      & other            & 66.66667 & 65.33333 & -1.33333 \\
tub                            & furniture        & 75.33333 & 73.33333 & -2       \\
Shih-Tzu                       & dog              & 92.66667 & 90.66667 & -2       \\
cauliflower                    & vegetable        & 94       & 92       & -2       \\
komondor                       & dog              & 91.33333 & 88.66667 & -2.66667 \\
English foxhound               & dog              & 36.66667 & 34       & -2.66667 \\
vizsla                         & dog              & 70.66667 & 68       & -2.66667 \\
kuvasz                         & dog              & 87.33333 & 83.33333 & -4    \\  
\bottomrule
\end{tabular}
\end{table}
